A Simple and Efficient Algorithm for Nonlinear Model Predictive Control

We present PANOC, a new algorithm for solving optimal control problems arising in nonlinear model predictive control (NMPC). A usual approach to this type of problems is sequential quadratic programming (SQP), which requires the solution of a quadratic program at every iteration and, consequently, inner iterative procedures. As a result, when the problem is ill-conditioned or the prediction horizon is large, each outer iteration becomes computationally very expensive. We propose a line-search algorithm that combines forward-backward iterations (FB) and Newton-type steps over the recently introduced forward-backward envelope (FBE), a continuous, real-valued, exact merit function for the original problem. The curvature information of Newton-type methods enables asymptotic superlinear rates under mild assumptions at the limit point, and the proposed algorithm is based on very simple operations: access to first-order information of the cost and dynamics and low-cost direct linear algebra. No inner iterative procedure nor Hessian evaluation is required, making our approach computationally simpler than SQP methods. The low-memory requirements and simple implementation make our method particularly suited for embedded NMPC applications.

==> TeX/Alg/BAD.tex <==
\begin{algorithmic}[1]
	\Inputs
		\(x_0\in\R^n\),~
		\(u=(\range{u_0}{u_{N-1}})\)%
	\Outputs
		\(\ell(u)\),~
		\(\nabla\ell(u)\)%
	\STATE
		\(\ell(u)\gets 0\)%
	\FOR{\(n=\range{0}{N-1}\)}
		\def\spaceWell#1#2{\fillwidthof[c]{x_{n+1}}{#1}\fillwidthof[c]{{}\gets{}}{{}#2{}}}
		\STATE
			\(\spaceWell{x_{n+1}}=f_n(x_n,u_n)\)
		\STATE
			\(\spaceWell{\ell(u)}\gets\ell(u)+\ell_n(x_n,u_n)\)
	\ENDFOR{}
	\def\spaceWell#1#2{\fillwidthof[c]{\ell(u)}{#1}\fillwidthof[c]{{}\gets{}}{{}#2{}}}
	\STATE
		\(\spaceWell{\ell(u)}\gets\ell(u)+\ell_N(x_N)\)
	\STATE
		\(\spaceWell{p_N}=\nabla \ell_N(x_N)\)
	\FOR{\(n=\range{N-1}{0}\)}
		\def\spaceWell#1#2{\fillwidthof[r]{\nabla\!_{u_n}\!\ell(u)}{#1}\fillwidthof[c]{{}\gets{}}{{}#2{}}}
		\STATE
			\(\spaceWell{p_n}=\nabla_{x_n} f_n(x_n,u_n)p_{n+1}+\nabla_{x_n}\ell_n(x_n,u_n)\)
		\STATE
			\(\spaceWell{\nabla\!_{u_n}\!\ell(u)}=\nabla_{u_n} f_n(x_n,u_n)p_{n+1}+\nabla_{u_n} \ell_n(x_n,u_n)\)
	\ENDFOR{}
 \end{algorithmic}


==> TeX/preamble_Panos.tex <==
\let\proof\relax
\let\endproof\relax
\usepackage{amsthm}

\usepackage[utf8]{inputenc}
\usepackage{url,bm}
%\usepackage{mathabx}
\usepackage{graphics}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{tikz}
\usepackage{pgfplots}

\usetikzlibrary{pgfplots.groupplots,matrix}
%\tikzexternalize[prefix=tikz/]

\usepackage{caption}
\usepackage{subcaption}

%\usepackage[noend]{algorithmic}
\usepackage{algpseudocode}
\usepackage{algorithm}
%\usepackage[ruled,commentsnumbered]{algorithm2e}
\usepackage{cite}
\usepackage{mathrsfs}
\usepackage[unicode=true,pdfusetitle, bookmarks=true,bookmarksnumbered=false,bookmarksopen=false, breaklinks=false,pdfborder={0 0 0},backref=false,colorlinks=true,linkcolor=blue]{hyperref}
\usepackage{enumerate}
\usepackage[mathscr]{euscript}
 \usepackage[all]{hypcap} % to help hyperref lead to right place
\usepackage{cleveref}
%\usepackage{ifpdf}
\usepackage{color}
%\ifpdf
%\usepackage[pdftex]{graphicx}
%\else
%\usepackage{graphicx}
%\fi



\newcommand{\bld}[1]{\boldsymbol{#1}}

\newcommand{\lb}[1]{ {\underline {#1}}} %lower bounds
\newcommand{\ub}[1]{ {\overline {#1}}} %upper bounds
\newcommand{\stsum}[1]{\displaystyle\sum\limits #1} % nice sum
\newcommand{\pte}[1]{ ~\mbox{\color{red} #1}} % pano's comments in equations
\newcommand{\pt}[1]{{\color{red} #1}} % pano's comments
\newcommand{\smallmat}[1]{\left[ \begin{smallmatrix}#1 \end{smallmatrix} \right]}
\newcommand{\eqdef}{\triangleq}
\newcommand{\cprod}{\ell_{\mathrm{prod}}}
\newcommand{\st}{\mathrm{s.t.}}
\renewcommand{\null}{\mathop{\rm null}\nolimits}
\newcommand{\ri}{\mathop{\rm ri}\nolimits}
\newcommand{\cl}{\mathop{\rm cl}\nolimits}
\newcommand{\dom}{\mathop{\rm dom}\nolimits}
\newcommand{\gph}{\mathop{\rm gph}\nolimits}
\newcommand{\conv}{\mathop{\rm conv}\nolimits}
\newcommand{\cone}{\mathop{\rm cone}\nolimits}
\newcommand{\rint}{\mathop{\rm rint}\nolimits}
\newcommand{\lev}{\mathop{\rm lev}\nolimits}
\newcommand{\aff}{\mathop{\rm aff}\nolimits}
\newcommand{\supp}{\mathop{\rm supp}\nolimits}
\newcommand{\Int}{\mathop{\rm int}\nolimits}
\newcommand{\id}{\mathop{\rm Id}\nolimits}
\newcommand{\dist}{\mathop{\rm dist}\nolimits}
\newcommand{\diag}{\mathop{\rm diag}\nolimits}
\newcommand{\blkdiag}{\mathop{\rm blkdiag}\nolimits}
\newcommand{\df}{\mathrm{d}f}
\newcommand{\ddf}{\mathrm{d}^2f}
\newcommand{\prox}{\mathop{\rm prox}\nolimits}
\newcommand{\fix}{\mathop{\rm Fix}\nolimits}
\newcommand{\ddiag}{\mathop{\rm diag}\nolimits}
\newcommand{\sign}{\mathop{\rm sign}\nolimits}
\newcommand{\soft}{\mathop{\rm soft}\nolimits}
\newcommand{\lmigeq}{\succcurlyeq}
\newcommand{\minimize}{\operatorname{minimize}}  
\newcommand{\maximize}{\operatorname{maximize}}  
% Sets
\renewcommand{\Re}{{\rm{I\!R}} }
\newcommand{\Rinf}{\overline{\rm I\!R}}
\newcommand{\Nn}{{\rm{I\!N}}}
\newcommand{\Bb}{{\rm I\!B} }
% Hilbert spaces
\newcommand{\ZZ}{\mathcal Z}
\newcommand{\HH}{\mathcal H}
\newcommand{\KK}{\mathcal K}
% set-valued mappings
\newcommand{\rra}{\rightrightarrows}


\newcommand{\sol}{\mathop{\rm SOL}\nolimits}
\newcommand{\zer}{\mathop{\rm zer}\nolimits}
\newcommand{\gra}{\mathop{\rm gra}\nolimits}

%\newcommand{\argmin}{\mathop{\rm arg\ min}\nolimits}
%\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmin}{\arg\!\min}
%\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\stt}{\rm subject\ to}



\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{conclusion}[theorem]{Conclusion}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{criterion}[theorem]{Criterion}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}{Remark}


\newtheorem{thm}{Theorem}
\newtheorem{lem}{Lemma}
\newtheorem{prop}{Proposition}
\newtheorem{coro}{Corollary}

%\theoremstyle{remark}
\newtheorem{rem}{Remark}

%\theoremstyle{definition}
\newtheorem{ass}{Assumption}
\newtheorem{alg}{Algorithm}
\newtheorem{deff}{Definition}


\crefname{thm}{Thm.}{Thm.}
\Crefname{thm}{Theorem}{Theorems}
\crefformat{thm}{#2Thm. #1#3}
\Crefformat{thm}{#2Theorem #1#3}
\crefmultiformat{thm}{#2Thm. #1#3}{ and #2#1#3}{, #2#1#3}{ and #2#1#3}
\Crefmultiformat{thm}{#2Theorems #1#3}{ and #2#1#3}{, #2#1#3}{ and #2#1#3}

\crefname{prop}{Prop.}{Prop.}
\Crefname{prop}{Proposition}{Propositions}
\crefformat{prop}{#2Prop. #1#3}
\Crefformat{prop}{#2Proposition #1#3}
\crefmultiformat{prop}{#2Prop. #1#3}{ and #2#1#3}{, #2#1#3}{ and #2#1#3}
\Crefmultiformat{prop}{#2Propositions #1#3}{ and #2#1#3}{, #2#1#3}{ and #2#1#3}


\crefname{coro}{Cor.}{Cro.}
\Crefname{coro}{Corollary}{Corollaries}
\crefformat{coro}{#2Cor. #1#3}
\Crefformat{coro}{#2Corollary #1#3}
\crefmultiformat{coro}{#2Cor. #1#3}{ and #2#1#3}{, #2#1#3}{ and #2#1#3}
\Crefmultiformat{coro}{#2Corollaries #1#3}{ and #2#1#3}{, #2#1#3}{ and #2#1#3}

\crefname{lem}{Lem.}{Lem.}
\Crefname{lem}{Lemma}{Lemmas}
\crefformat{lem}{#2Lem. #1#3}
\Crefformat{lem}{#2Lemma #1#3}
\crefmultiformat{lem}{#2Lem. #1#3}{ and #2#1#3}{, #2#1#3}{ and #2#1#3}
\Crefmultiformat{lem}{#2Lemmas #1#3}{ and #2#1#3}{, #2#1#3}{ and #2#1#3}

\crefname{algorithm}{Alg.}{Alg.}
\Crefname{algorithm}{Algorithm}{Algorithms}
\crefformat{algorithm}{#2Alg. #1#3}
\Crefformat{algorithm}{#2Algorithm #1#3}
\crefmultiformat{algorithm}{#2Alg. #1#3}{ and #2#1#3}{, #2#1#3}{ and #2#1#3}
\Crefmultiformat{algorithm}{#2Algorithms #1#3}{ and #2#1#3}{, #2#1#3}{ and #2#1#3}

\crefname{rem}{Rem.}{Rem.}
\Crefname{rem}{Remark}{Remarks}
\crefformat{rem}{#2Rem. #1#3}
\Crefformat{rem}{#2Remark #1#3}
\crefmultiformat{rem}{#2Rem. #1#3}{ and #2#1#3}{, #2#1#3}{ and #2#1#3}
\Crefmultiformat{rem}{#2Remarks #1#3}{ and #2#1#3}{, #2#1#3}{ and #2#1#3}

\crefname{ass}{Ass.}{Ass.}
\Crefname{ass}{Assumption}{Assumption}
\Crefformat{ass}{#2Assumption #1#3}
\Crefmultiformat{ass}{#2Assumptions #1#3}{ and #2#1#3}{, #2#1#3}{ and #2#1#3}

\crefname{deff}{Def.}{Def.}
\Crefname{deff}{Definition}{Definition}
\crefformat{deff}{#2Def. #1#3}
\Crefformat{deff}{#2Definition #1#3}


\Crefname{section}{Section}{Sections}
\Crefformat{section}{#2Section #1#3}
\Crefmultiformat{section}{#2Sections #1#3}{ and #2#1#3}{, #2#1#3}{ and #2#1#3}


\Crefname{enumi}{Assumption}{Assumptions}
\Crefformat{enumi}{Assumption #21(#1)#3}
\Crefmultiformat{enumi}{Assumptions (#2#1#3)}{ and (#2#1#3)}{, (#2#1#3)}{ and (#2#1#3)}
\crefrangeformat{enumi}{Assumptions ~(#3#1#4) to~(#5#2#6)}

\Crefname{figure}{Figure}{Figures}
\Crefformat{figure}{#2Figure #1#3}
